V*: Guided Visual Search as a Core Mechanism in Multimodal LLMs

When we look around and perform complex tasks, how we see and selectively process what we see is crucial. However, the lack of this visual search mechanism in current multimodal LLMs (MLLMs) hinders their ability to focus on important visual details, especially when handling high-resolution and visually crowded images. To address this, we introduce V*, an LLM-guided visual search mechanism that employs the world knowledge in LLMs for efficient visual querying. When combined with an MLLM, this mechanism enhances collaborative reasoning, contextual understanding, and precise targeting of specific visual elements. This integration results in a new MLLM meta-architecture, named Show, sEArch, and TelL (SEAL). We further create V*Bench, a benchmark specifically designed to evaluate MLLMs in their ability to process high-resolution images and focus on visual details. Our study highlights the necessity of incorporating visual search capabilities into multimodal systems. The code is available https://github.com/penghao-wu/vstar.

==> sec/3_method.tex <==
\section{Method}
\label{sec:method}

\begin{figure*}[ht]
\centering
\includegraphics[width=\linewidth]{figures/pipeline_v2.pdf}
\caption{An instantiation of the proposed SEAL framework. The left part is the VQA LLM which takes all the information in the VWM to answer questions. The right part demonstrates the process of the V$^*$ visual search algorithm.}
\label{fig:framework}
\end{figure*}

Our proposed SEAL framework is a general meta-architecture for MLLMs. It is comprised of a VQA LLM and a visual search model which collaborate and interact through the visual working memory (VWM). An illustration of the SEAL framework is shown in Fig~\ref{fig:framework}. In this work, we provide a simple instantiation of the SEAL framework to validate its effectiveness and choose the LLaVA-7B structure as the MLLM in the SEAL framework.
We will first elaborate on the model structures, and then introduce the training data curation process for each of these two parts.
% We now elaborate on the model structures of each of these two parts. The training data curation process and the training details are provided in the Supplementary.
\subsection{VQA LLM with Visual Working Memory}
\subsubsection{Model Structure}
Current MLLMs usually have three components: a vision encoder, a projection module, and an LLM. While different models may have different projection modules (\eg Resampler \cite{flamingo,otter,wang2023makes}, QFormer \cite{blip2, InstructBLIP}, and linear layer \cite{llava, chen2023shikra}) and insert the projected vision tokens into the input layer \cite{blip2,InstructBLIP,minigpt4,llava} or middle cross-attention layers \cite{flamingo,otter} of the LLM, most of them adopt the pre-trained CLIP vision transformer as their vision encoder. When tackling higher-resolution images or images with abundant information, the visual features extracted by the vision encoder may not contain certain information needed to answer the question.

\begin{algorithm}
% \scriptsize
\DontPrintSemicolon
\SetAlgoNoEnd
\caption{SEAL Working Pipeline}
\label{algo:SEAL}
\SetKwFunction{FMain}{SEALVQA}
\SetKwFunction{VS}{Visual Search}
\SetKwFunction{VQA}{VQALLM}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\FMain{$I$, $T$, $\delta$}}{
    list of needed target objects $L$ $ \leftarrow$  \VQA{$I$, $T$}\;
    Initialize VWM \;
    VWM.add($I$),
    VWM.add($T$) \;
    \For{target in $L$}{
        Priority queue $q$\;
        $q.add(($I$, \infty))$\;
        search result $ \leftarrow$ \VS{$q$, $s$, $\delta$}\;
        \If{search result is None}{
            VWM.add("\{target\} not existent in the image")
        }
        \Else{
            Cropped the object patch from $I$\;
            VWM.add("\{target\} $<$object patch$>$ at location $[x1, y1, x2, y2]$")\;
        }
    }
    response $ \leftarrow$  \VQA{VWM}\;
    \KwRet response\;
}    
\end{algorithm}

To tackle this problem, our model first actively reasons about whether the initial visual feature from the vision encoder is enough to answer the question. If not, it explicitly lists all the needed but missing information in the format of a list of target objects. Then, it initializes a VWM. The VWM has four blocks, the $<$question$>$ block contains the initial textual question; the $<$global image$>$ block contains the initial global image; the $<$searched targets$>$ block is designed to contain all the target object crops after search; and the $<$target location$>$ block would contain the coordinates of the searched targets. Next, the visual search model searches over the image and localizes each required target. A region containing the retrieved target is then cropped from the whole image and filled in the VWM together with the coordinates of the target. After that, the VQA LLM processes the information contained in the VWM and generates the response accordingly. The working pipeline of the SEAL framework is illustrated in Algorithm~\ref{algo:SEAL}.

 In this work, we choose the CLIP ViT-L-14 model as the vision encoder with input resized and padded to $224^2$, and use it to process both the initial image and the crops of searched targets. To further project the visual features to become the input of the LLM, we consider two kinds of projection modules (\ie the linear layer and the resampler). The linear layer projection module keeps the number of visual tokens from the vision encoder while the cross-attention based resampler projection reduces the number of tokens (\ie 256 to 32). To avoid excessive long tokens and help the language model better focus on the most critical information, we have designed a simple scheme to flexibly switch between these two projection modules. Specifically, when the input only includes the initial image feature without any searched targets, the simple linear layer projection is applied to keep all the visual tokens. When there are one or two searched targets in the VWM, we assume that answering the question requires the model to focus on the searched targets, therefore, we use the linear layer projection to project the visual features of the searched targets and adopt the resampler to condense the original image features. As for other cases where the VWM contains more searched targets, we use the resampler as the projection module for all visual features to relieve the computational burden.
% Finally, the input sequence to the language model is: 
% \begin{tcolorbox}[enhanced]
% \texttt{<Image> \\
% Additional visual information to focus on: \\ 
% \{Target Object 1's Name\} <Object> at location [x1, y1, x2, y2]; \\
% \{Target Object 2's Name\} <Object> at location [x1, y1, x2, y2]; \\
% $\cdots$ \\
% Question}
% \end{tcolorbox}, where \texttt{<Image>} is the feature tokens of the image and \texttt{<Object>} is the feature tokens of the target object stored in the visual buffer. And the vision language model can then focus on the key information retrieved by the visual search process to make responses. \todo{sx:this seems too big; wasting space}


\subsection{V$^*$: LLM-guided Visual Search}
\subsubsection{Problem Formulation}
Similar to the referring expression comprehension (REC) task, the goal of visual search is to localize the certain object in the image described by a textual referring expression. However, different from the REC task which is limited to images within a certain size, our task generalizes to images of any resolution and a search over the image might be required to finally locate the described object. Therefore, a good visual search algorithm also needs to locate the final target efficiently in as little time as possible.

\subsubsection{Model Structure}
Given a high-resolution image, it is likely that the target object can not be accurately identified and localized when just viewing the whole image as a miniature. To tackle this problem, one intuitive solution is dividing the image into fixed-size small sub-images and exhaustively conducting the localization on each sub-image, which is commonly used in the field of aerial image detection and whole slide image analysis  \cite{ozge2019power, chen2022scaling}. However, this simple strategy becomes prohibitively inefficient when considering the case of any resolution images. 


% To find a specific object in a large image, humans would first go to specific areas where we believe there exists a higher possibility of finding the target according to common sense knowledge \eg flags are more likely to appear on the roof of buildings and plates are more likely to be found on tables. This ability enables humans to find the targets much more efficiently. 

As humans' visual search process is guided by contextual scene guidance and top-down feature guidance, we adopt similar ideas to design the visual search model in the V$^*$ algorithm utilizing an MLLM which encapsulates a mass of common sense knowledge about the world. In order to complete the whole searching process, we also equip the MLLM with localization ability similar to \cite{LISA, contextDET}.  

Our visual search model consists of an MLLM and a localization module with an image backbone and two decoders, \ie a target localization decoder $D_{tl}$ and a search cue localization decoder $D_{cl}$. The MLLM has additional localization ability with a localization token \texttt{<LOC>} added to its vocabulary. Given an image and a textual expression of an object or region, the textual expression is first transformed into a fixed-format instruction (\ie "Please locate the \texttt{[object]} in the image.") and then fed into the MLLM together with the image. The MLLM outputs the localization token \texttt{<LOC>} containing contextual and location-related information of the queried textual expression. We extract the last layer embedding of this token $\bm{v}_{loc}$ and process it with two separate MLPs to $\bm{v}_{tl}$ and $\bm{v}_{cl}$ for further uses. The image features obtained from the image backbone are then combined with $\bm{v}_{tl}$ and $\bm{v}_{cl}$ and are processed by the two decoders to output coordinates plus confidence scores and heatmap respectively. The detailed model structures of $D_{tl}$ and $D_{cl}$ are shown in the Supplementary.


\subsubsection{Search Algorithm}

With this visual search model, our V$^*$ algorithm works as follows. Given an image and a textual expression of the target object, the MLLM first attempts to locate the target. In this step, $\bm{v}_{loc}$ corresponding to the target object generated by the MLLM is fed to both $D_{tl}$ and $D_{cl}$ to obtain the coordinates with confidence score and the heatmap. When no object is located in the current image (the confidence score is smaller than a pre-defined threshold), we scrutinize the heatmap for possible target-specific cues. 

The heatmap highlights regions that look similar to the queried target object, representing the target-specific cue. When the target-specific cue is prominent (\ie the maximum value of the heatmap is larger than a threshold $\delta$), we use it as guidance for the search. Otherwise, we ask the MLLM what is the most likely location of the target object in the image. This requires the MLLM to utilize its common sense knowledge and combine it with the image context to give us the contextual cue about the target. After getting an expression indicating the region where the target object is likely to be found, we prompt the MLLM to locate this expression with the $D_{cl}$ decoder and get the heatmap corresponding to the contextual cue. 

Then, we split the current image into smaller sub-images and assign them scores indicating their priorities to be explored based on the target-specific cue heatmap or the contextual cue heatmap. Based on the priorities, the sub-images are cropped and processed in turn. This recursive process continues until we successfully locate the target object or the current image patch is smaller than a pre-defined threshold. The overall process of the V$^*$ algorithm is illustrated in Algorithm~\ref{alg:visual search}.

Our LLM-guided visual search algorithm V$^*$ shares some similarities with the informed search algorithm A$^*$. The A$^*$ search algorithm is a path search algorithm that finds the shortest path between a start and a goal node using a heuristic to estimate the cost. The LLM-guided visual search algorithm of our V$^*$ can viewed as a special case of A$^*$ where the sub-images are viewed as nodes and $g(n)$ is a positive constant for all $n$ and the heuristic function $h(n)$ is $-1\times$ (score calculated from the heatmap). However, the goal of the A$^*$ search algorithm is to find a path with the minimum cost from the start to the goal, while in our case, we only care about the total number of steps needed to find the goal.


\begin{algorithm}
\DontPrintSemicolon
\SetAlgoNoEnd
% \scriptsize
\caption{\emph{V}$^*$: LLM-guided Visual Search}\label{alg:visual search}
\SetKwFunction{FMain}{Visual Search}
\SetKwFunction{VSM}{VisualSearchModel}

\SetKwProg{Fn}{Function}{:}{}
\Fn{\FMain{$q$, $s$, $\delta$}}{
    Current image $I_p$ = $q.pop()$\;
    localization result, heatmap $ \leftarrow$ \VSM{instruction="Please locate the $s$ in the image.", image=$I_p$}\;
    
    \If{localization result is not None}{ 
        \KwRet localization result\;
    }
    \If{heatmap.max() $< \delta$ }{
        contextual cue $ \leftarrow$ \VSM{instruction="What is the most likely location of the $s$ in the image?", image=$I_p$}
        \;
        \_ , heatmap $ \leftarrow$ \VSM{instruction="Please locate the 'contextual cue' in the image.", image=$I_p$} \;
    }
    Divide $I_p$ into sub-images, calculate the priority for each sub-image based on the heatmap, and add (sub-image, priority) pairs to $q$. \;
    \While{$q$ is not empty}{
        search result $ \leftarrow$ \FMain{$q$, $s$, $\delta$} \;
        \If{search result is not None}{
            \KwRet search result\;
        }
    }
    \KwRet None
}
\end{algorithm}
% % Up to now, it is just the same as the common practice for open-vocabulary object detection or referring expression comprehension. However, considering an image of arbitrarily large resolution, it is very likely that the target object can not be located when we resize the whole image to a small size one on the first try.
% When no object is located in the current image (the confidence score is smaller than a pre-defined threshold), we scrutinize the heatmap for possible target-specific cues. The score of each pixel on the heatmap denotes the likelihood that it belongs to the target area. Therefore, the heatmap highlights regions that look similar to the queried target object, representing the target-specific cue. When the maximum value of the heatmap is larger than a threshold $\sigma$, we say this target-specific cue is prominent and thus use it as guidance for the search.
% When the target-specific cue is not prominent, namely, there are no objects or regions sharing similar visual characteristics with the target object, 
% Otherwise, we ask the multimodal LLM what is the most likely location of the target object in the image. This requires the multimodal LLM to utilize its common sense knowledge and combine it with the image context to give us the contextual cue about the target. After getting an expression indicating the region where the target object is likely to be found, we prompt the multimodal LLM to locate this expression with the $D_{cl}$ decoder and get the heatmap corresponding to the contextual cue. Then, we split the current image into smaller sub-images and assign them scores indicating their priorities to be explored based on the target-specific cue heatmap or the contextual cue heatmap. Based on the priorities, the sub-images are cropped and processed in turn. This recursive process continues until we successfully locate the target object from $D_{tl}$ or the current image patch is smaller than a pre-defined threshold. The overall LLM-guided visual search process is illustrated in Algo~\ref{alg:visual search}.


